Yankee Swap: a Fast and Simple Fair Allocation Mechanism for Matroid Rank Valuations

We study fair allocation of indivisible goods when agents have matroid rank valuations. Our main contribution is a simple algorithm based on the colloquial Yankee Swap procedure that computes provably fair and efficient Lorenz dominating allocations. While there exist polynomial time algorithms to compute such allocations, our proposed method improves on them in two ways. (a) Our approach is easy to understand and does not use complex matroid optimization algorithms as subroutines. (b) Our approach is scalable; it is provably faster than all known algorithms to compute Lorenz dominating allocations. These two properties are key to the adoption of algorithms in any real fair allocation setting; our contribution brings us one step closer to this goal.

==> dump.tex <==
\subsection{Other Notions of Fairness}
\todo{Trim this down to be consistent with the introduction}
There are several other popular notions of fairness and efficiency. We list them here:

\begin{description}
    \item[\MAXUSW] An allocation $X$ is said to maximize {\em utilitarian social welfare} if it maximizes $\sum_{i \in N} v_i(X_i)$.
    \item[\MNW] An allocation $X$ is said to maximize {\em Nash social welfare} if it maximizes $\prod_{i \in N} v_i(X_i)$.
    \item[\MMS] An agent's {\em maxmin share} is defined as the utility they would obtain if they divided the goods into $n$ bundles and picked the worst of these bundles. More formally, 
    \begin{align*}
        \MMS_i = \min_{X_j \in X} \max_{X = (X_1, X_2, \dots, X_n)} v_i(X_j))
    \end{align*} 
    An allocation is $c\MMS$ if it guarantees every agent $i \in N$ utility of at least $c \MMS_i$. 
    \item[Min-squared] A \MAXUSW{} allocation $X$ is min-squared if it minimizes $\sum_{i \in N}$ $v_i(X_i)^2$ among all the allocations which are \MAXUSW.
    \item[Envyfreeness] An allocation $X$ is said to be envy free if for all $i, j \in N$, $v_i(X_i) \ge v_i(X_j)$ i.e. no agent values another agent's bundle over their own. However, this is not always achievable --- consider a problem instance with two agents and one good. A few relaxations have been proposed and studied in the literature: 
    \begin{inparaenum}[(a)]
        \item {\em EF1}: $X$ is EF1 if for every pair of agents $i, j \in N$, there is always a good $g \in X_j$ such that $v_i(X_i) \ge v_i(X_j - g)$.
        \item {\em EFX}: $X$ is EFX if for every pair of agents $i, j \in N$, for any $g \in X_j$, we have $v_i(X_i) \ge v_i(X_j - g)$.
        \item {\em Stochastic envyfreeness}: A randomized allocation $X$ is stochastic envy free if for all pairs of agents $i, j \in N$ and every value $t$, we have $\Pr[v_i(X_i) \ge t] \ge \Pr[v_i(X_j) \ge t]$.
        \item {\em Ex-ante envyfreeness}: A randomized allocation $X$ is ex-ante envy free if for all pairs of agents $i, j \in N$, we have $\E[v_i(X_i)] \ge \E[v_i(X_j)]$. EFX and stochastic envyfreeness are stronger notions than EF1 and ex-ante envyfreeness respectively.
    \end{inparaenum}
    \item[Proportionality] An allocation $X$ is proportional if for all agents $i \in N$, $v_i(X_i) \ge \frac{v_i(G)}{n}$. Like envyfreeness, proportionality is also impossible to guarantee: again, consider the instance with two agents and one good. There have been two prominent relaxations of proportionality proposed in the literature: 
    \begin{inparaenum}[(a)]
        \item {\em PROP1}: $X$ is PROP1 if for every agent $i \in N$, there exists a good $g \in G$ such that $v_i(X_i+ g) \ge  \frac{v_i(G)}{n}$.
        \item {\em Ex-ante proportionality}: A randomized allocation $X$ is said to be ex-ante proportional if for all agents $i \in N$, $\E[v_i(X_i)] \ge \frac{v_i(G)}{n}$.
    \end{inparaenum}
    \item[Lorenz dominating] An allocation $X$ is said to be Lorenz-dominating if for all other allocations $Y$ and every $k \in [n]$, we have $\sum_{j = 1}^k u^X_j \ge \sum_{j = 1}^k u^Y_j$ where $\vec u^X$ and $\vec u^Y$ are the sorted utility vectors of $X$ and $Y$ respectively.
\end{description}
Apart from fairness and efficiency, an important property of algorithms which compute fair allocations is {\em strategyproofness} i.e. no agent can gain by misreporting their valuation function.

\citet{Babaioff2021Dichotomous} use the concept of Lorenz dominating allocations but use auxiliary goods to create a priority ordering between the agents. 
Given a priority ordering $\pi: N \mapsto [n]$, they add $n$ goods $A = \{a_1, a_2, \dots, a_n\}$ to the problem instance where each agent $i$ values $a_i$ at $\frac{\pi(i)}{n^2}$ and the other goods in $A$ at $0$.

More formally, the create a new fair allocation problem instance with the set of agents $N$ and the set of goods $G \cup A$ where each agent $i$ has the following valuation function $v'_i$:
\begin{align*}
    v'_i(S) = v_i(S \cap G) +\frac{\pi(i)}{n^2}|S \cap \{a_i\}|
\end{align*}
The goods in $A$ do not exist in reality and serve only to break ties between agents. After computing a Lorenz dominating allocation for this artificial problem instance, they remove the goods from $A$ and allocate the goods from $G$ to the agents according to the computed allocation. They refer to this allocation as a Lorenz dominating allocation with respect to the priority order $\pi$.

\citet{Babaioff2021Dichotomous} show that these Lorenz dominating allocation with respect to any ordering $\pi$ is \MNW, \MAXUSW, Min-squared, leximin, EFX and $(1/2)\MMS$. They also show that these allocations can be computed in polynomial time.
\begin{theorem}[\citet{Babaioff2021Dichotomous}]
Whena agents have MRF valuations, lorenz dominating allocations with respect to any ordering $\pi$ are \MNW, \MAXUSW, Min-squared, leximin, EFX and $(1/2)\MMS$. They can also be computed in polynomial time. When agents have additive valuations, these lorenz dominating allocation are $\MMS$ as well.
\end{theorem}

They also propose a mechanism which chooses the priority order $\pi$ uniformly at random. Apart from the guarantees offered by the above theorem, they show that the mechanism is strategy proof and results in a random allocation which is stochastically envy-free and ex-ante proportional. Their mechanism is called randomized prioritized egalitarian (RPE) and works as follows: 
\begin{enumerate}[(a)]
    \item Choose a priority order $\pi$ uniformly at random
    \item Ask each agent to report their preferences. If an agent's reported preferences are not an MRF, assume their valuation for every bundle is $0$.
    \item Compute a Lorenz dominating allocation for the reported preferences with respect to the priority order $\pi$.
\end{enumerate}

\begin{theorem}[\citet{Babaioff2021Dichotomous}]
The RPE mechanism is strategy proof and when agents report preferences truthfully, results in an allocation which is stochastically envy-free and ex-ante proportional.
\end{theorem}

To add to this cornucopia of positive results, we show that Lorenz dominating allocations with respect to any priority ordering $\pi$ is PROP1 as well. Our proof uses the following simple observation.

\begin{obs}\label{obs:unallocated-marginal}
When agents have MRF valuations, let $X$ be a \MAXUSW{} allocation. Then, for any agent $i \in N$, we have $v_i(\bigcup_{j \in N} X_j) = v_i(G)$.
\end{obs}
\begin{proof}
Let $G' = \bigcup_{j \in N} X_j)$.
Since $X$ is utility maximizing, we must have that $\Delta_i(X_i, g) = 0$ for all $g$ in $X_0 = G \setminus G'$. If we have  $\Delta_i(X_i, g) = 1$ for some $g$ in $X_0$, we can move this good from $X_0$ to $X_i$ resulting in an allocation with higher utilitarian social welfare since this move will increase $i$'s utility.

Without loss of generality, let $X_0 = \{g_1, g_2, \dots, g_k\}$ and let $Z_j = \{g_1, g_2, \dots, g_j\}$. We have
\begin{align*}
    v_i(G) = v_i(G') + \sum_{j = 1}^k \Delta_i(G' \cup Z_{j-1}, g_j) \le v_i(G') + \sum_{j = 1}^k \Delta_i(X_i, g_j) = v_i(G') 
\end{align*}

Since marginal gains cannot be negative and $G' \subseteq G$, we have $v_i(G') \le v_i(G)$ as well. Combining the two inequalities gives us our result.
\end{proof}
\begin{prop}
When agents have MRF valuations, lorenz dominating allocations with respect to any priority ordering $\pi$ is PROP1
\end{prop}
\begin{proof}
Let $X$ be a non-redundant Lorenz dominating allocation. Consider the agent $i$. 
If $i$ does not envy any other agent, we have $v_i{X_i} \ge v_i(X_j)$ for all $j \in N$. Summing up the inequality for all $j \in N$, we get 
\begin{align*}
    n v_i(X_i) &\ge \sum_{j \in N} v_i(X_j) \ge v_i(\bigcup_{j \in N} X_j) = v_i(G)
\end{align*}
The second inequality results from the repeated application of \cref{obs:union-upperbound} and the final equality is implied by \cref{obs:unallocated-marginal}.

If $i$ envies some other agent (say $j$), then $|X_j| \ge |X_i| + 1$. If $|X_j| \le |X_i|$, then from \cref{obs:size-upperbound}, $v_i(X_j) \le |X_i| = v_i(X_i)$ --- $i$ does not envy $j$. Using similar arguments to that of \cref{obs:wlog-nonredundant} and \cref{obs:nonredundance-exchange}, we can show that there exists a good $g^*$ such that $\Delta_i(X_i, g^*) = 1$.

Since the allocation is EFX we must have $v_i(X_j) \le v_i(X_i) + 1$ for all $j \in N$. If $v_i(X_j) \ge v_i(X_i) + 2$, dropping any good will result in the reduction in value of at most $1$ due to binary marginal gains i.e. we get $v_i(X_j - g) \ge v_i{X_j} - 1 \ge v_i(X_i) + 1$, a contradiction since $i$ still envies $j$ after dropping a good. 

Combining the above two paragraphs, we get that $v_i(X_i + g^*) \ge v_i(X_j)$ for all $j \in N$. Summing up this inequality for all $j \in N$, we get 
\begin{align*}
    n v_i(X_i + g^{*}) &\ge \sum_{j \in N} v_i(X_j) \ge v_i(\bigcup_{j \in N} X_j) = v_i(G)
\end{align*}
The second inequality results from the repeated application of \cref{obs:union-upperbound} and the final equality is implied by \cref{obs:unallocated-marginal}. This completes the proof.
\end{proof}

We also show that Lorenz dominating allocations with respect to the ordering $\pi$ and prioritized leximin allocations with respect to the ordering $\pi$ are equivalent. This implies that our algorithm also possesses all the fairness properties discussed above and it can be used as a subroutine in RPE mechanism.

\todo{Continue writing from here}
\if 0
We denote the set of all agents which are present in at least one transfer path starting with $i$ under the allocation $X$ as $D_i(X)$. 
For a set of agents $S$, $D_S(X) = \bigcup_{i \in S}D_i(X)$.
Note that the fake agent $0$ may be in a transfer path and $D_i(X)$ for some $i$ and $X$. A transfer path involving agent $0$ is one where an agent takes an item from the unallocated pile $X_0$. These transfer paths play a crucial role in our analysis. This is mainly because, as we show in \cref{prop:demand-set-optimal}, if $X$ is non-redundant, no allocation has a better USW for the agents in $D_i(X)$ than $X$.

We prove two useful Lemmata.
\begin{lemma}\label{lem:demand-set-Pareto}
Let $X$ be a non-redundant allocation. When agents have MRF valuations, if there exists an allocation that has a higher USW for a particular set of agents $S \in N \cup \{0\}$, then there exists a non-redundant allocation which Pareto dominates $X$ for the set of agents $S \in N \cup \{0\}$.
\end{lemma}
\begin{proof}
Out of all the allocations which have a higher USW for a particular set of agents $S$, let $Y$ be a non-redundant allocation which maximizes $\sum_{j \in N \cup \{0\}}|X_j \cap Y_j|$. 
We argue that $Y$ Pareto dominates $X$ for the set of agents $S$.

Assume for contradiction that $Y$ does not Pareto dominate $X$ for the agents in $S$. 
Then we must have some agent $i \in S$ such that $|X_i| > |Y_i|$. 
Using the matroid exchange property there must exist some good in $g \in X_i \setminus Y_i$ such that $v_i(Y_i + g) > v_i(Y_i)$. This good $g$ is not in $Y_0$ by assumption since the allocation is non-redundant. Therefore this good belongs to another agent's allocation, say $Y_{i'}$. 
If $|X_{i'}| < |Y_{i'}|$, then we can create a new allocation $Z$ as follows
\begin{align*}
    Z_j = 
    \begin{cases}
        Y_j + g & j = i \\
        Y_j - g & j = i' \\
        Y_j & \text{otherwise.}
    \end{cases}
\end{align*}
It is easy to see that $Z$ has a weakly greater USW for the agents in $S$ than $Y$ and $\sum_{j \in  N \cup \{0\}} |X_j \cap Z_j| > \sum_{j \in  N \cup \{0\}} |X_j \cap Y_j|$. This contradicts our initial assumption on $Y$.
If $|X_{i'}| \ge |Y_{i'}|$. Again, by the matroid exchange property there must be a good $g' \in X_{i'} \setminus (Y_{i'} - g) = X_{i'} \setminus Y_{i'}$ such that $v_{i'}(Y_{i'} + g' - g) > v_{i'}(Y_{i'} - g)$. Assume this good is in $Y_{i''}$ $(i'' \ne i')$. 
By continuing this process with $i''$, we either end up in a cycle (for example, if $i'' = i$) or we have an acyclic sequence of agents $i \rightarrow i_1 \rightarrow i_2 \rightarrow \dots \rightarrow i_r$ such that $|Y_{i_r}| > |X_{i_r}|$.

If we obtain an acyclic sequence of agents $i \rightarrow i_1 \rightarrow i_2 \rightarrow \dots \rightarrow i_r$ such that $|Y_{i_r}| > |X_{i_r}|$, this is a transfer path for $i$ under the allocation $Y$ such that in every transfer, we can give an agent a good they had in $X$ and take away a good they did not have in $X$. This is true by construction. Let $Z$ be the allocation that results from making the above described transfer along this path. The allocation $Z$ has a weakly greater USW for the set of agents $S$ than $Y$ and we have $\sum_{j \in N \cup \{0\}} |X_j \cap Z_j| > \sum_{j \in N \cup \{0\}} |X_j \cap Y_j|$.

Similarly, if we have a cycle $i_1 \rightarrow i_2 \rightarrow \dots \rightarrow i_r \rightarrow i_1$, there exists a cyclic transfer such that at every transfer, we can give an agent a good they had in $X$ and take away a good they did not have in $X$. It is easy to see that the resulting allocation $Z$ provides each agent with the same utility as $Y$. This transfer also results in an allocation $Z$ such that $\sum_{j \in N \cup \{0\}} |X_j \cap Z_j| > \sum_{j \in N \cup \{0\}} |X_j \cap Y_j|$. 
\end{proof}

\begin{lemma}\label{lem:transfer}
Consider two non-redundant allocations $X$ and $Y$, if for some $i \in N \cup \{0\}$, $|X_i| \le |Y_i|$ and $X_i \nsubseteq Y_i$, then for every good $g \in X_i \setminus Y_i$, there exists a good $g' \in Y_i \setminus X_i$ such that $v_i(Y_i - g' + g) = v_i(Y_i)$ and $v_i(X_i + g' - g) = v_i(X_i)$
\end{lemma}
\begin{proof}
This proof has been adapted from \citet{brualdi1969bases}.
We switch to matroid speak for this proof. The matroid we refer to here is the one defined by the rank function $v_i$. We use the following properties of circuits for the proof.

\begin{lemma}[\citet{brualdi1969bases}]\label{lem:circuit-unique}
Given a matroid $(E, \cal I)$, if some set $S \in \cal I$ and there exists an element $e \in E$ such that $S + e \notin \cal I$, then $S + e$ contains a unique circuit.
\end{lemma}

\begin{lemma}[\citet{asche1966minimal}]\label{lem:circuit-intersection}
If $C_1$ and $C_2$ are circuits with $a \in C_1 \cap C_2$ and $b \in C_1 \setminus C_2$, there exists a circuit $C_3$ such that $b \in C_3 \subseteq (C_1 \cup C_2) - a$
\end{lemma}

In matroid terms, the goal of this proof is to find sets $Y_i + g - g'$ and $X_i - g + g'$ which are independent.
If $Y_i + g$ is independent, we are done. To find $g'$, we apply the exchange property --- there must be an element $g' \in (Y_i + g) \setminus X_i$ such that $X_i + g'$ is independent. If $Y_i + g$ is not independent, it must contain a unique circuit $C$ (\cref{lem:circuit-unique}). We must have $C \cap (Y_i \setminus X_i) \ne \emptyset$. If there exists $g'' \in C \cap (Y_i \setminus X_i)$ such that $X_i + g''$ is independent, we are done.

Otherwise, for all $g'' \in C \cap (Y_i \setminus X_i)$, $X_i + g''$ must contain a unique circuit (\cref{lem:circuit-unique}). If none of these circuits contain $g$, then we can repeatedly apply \cref{lem:circuit-intersection} to create a circuit which contains $g$ but is contained in $X_i$ --- a contradiction. Therefore, there must be a $g' \in C \cap (Y_i \setminus X_i)$ such that the unique circuit contained in $X_i \cup g'$ contains $g$. From this, we have that $Y_i - g' + g$ and $X_i -g + g'$ are independent sets. This completes the proof.
\end{proof}
% \begin{proof}
% Start with $(X_i \cap Y_i) + g$. This is independent in the matroid defined by $v_i$ since it is a subset of $X_i$. Now repeatedly apply the exchange property using $Y_i$ till you get a set of size $|Y_i|$. There has to be a good that $Y_i$ has that this new set does not have. They're both independent and of the same size, so we're done.
% \end{proof}

\begin{prop}\label{prop:demand-set-optimal}
Let $X$ be any non redundant allocation. There exists no other allocation $Y$ such that achieves a higher USW for the set of agents $D_S(X)$ for any $S \subseteq N \cup \{0\}$.
\end{prop}
\begin{proof}
% Right now, I have only added the proof for $D_i(X)$ for any $i \in N$. The extension is fairly easy to see. Will add it later.

Assume for contradiction there is a non-redundant allocation $Y$ with higher USW for the set of agents $D_S(X)$ for some $S \subseteq N \cup \{0\}$. From \cref{lem:demand-set-Pareto}, we can assume without loss of generality that $Y$ Pareto dominates $X$ for the set of agents $D_S(X)$. Further assume that, of all the allocations which Pareto dominate $X$ for the set of agents $D_i(X)$, $Y$ maximizes $\sum_{j \in N \cup \{0\}} |X_j \cap Y_j|$. 
Let $X_S = \bigcup_{j \in D_S(X)} X_j$ be the set of goods allocated to agents in $D_S(X)$.

If $X_j \subseteq Y_j$ for all $j \in D_S(X)$, then this proof is trivial. There must be some agent $i'$ such that $Y_{i'} \setminus X_{i'} \ne \emptyset$. Let $g$ be an arbitrary good in $Y_{i'} \setminus X_{i'}$. $g$ is not in $X_S$ since all the agents in $D_S(X)$ received supersets of their allocations in $X$. Let the agent who has $g$ in $X$ be $i''$. There must be a transfer path from some agent $i \in S$ to $i'$ by definition since $i'$ in $D_S(X)$. This transfer path can be extended to include an edge from $i'$ to $i''$ since whatever good $i'$ gives away in the initial path, it can take $g$ from $i''$ and retain its original valuation. This means there is a transfer path from $i$ to $i''$ which is a contradiction since $i'' \notin D_S(X)$.

We now move to the case where $X_j \nsubseteq Y_j$ for some $j \in D_S(X)$. Since $Y$ Pareto dominates $X$ for the set of agents $D_S(X)$, there must exist an agent $i_1 \in D_S(X)$ such that $v_{i_1}(Y_{i_1}) > v_{i_1}(X_{i_1})$. By the matroid exchange property, there must exist a good $g \in Y_{i_1} \setminus X_{i_1}$ such that $v_{i_1}(X_{i_1} + g) > v_{i_1}(X_{i_1})$. Let this good belong to some other agent $i_2$. By the same logic used in the previous paragraph, $i_2 \in D_S(X)$. We create an allocation $Z$ as a copy of $Y$ but move $g$ from $i_1$ to $i_2$. If $v_{i_2}(Z_{i_2}) > v_{i_2}(Y_{i_2})$, then we are done because we have created a Pareto dominant allocation $Z$ such that $\sum_{j \in N \cup \{0\}} |X_j \cap Z_j| > \sum_{j \in N \cup \{0\}} |X_j \cap Y_j|$. Otherwise there must be some good $g' \in Y_{i_2}$ that $i_2$ can give away such that $v_{i_2} (Y_{i_2} + g - g') = v_{i_2}(Y_{i_2})$ and $v_{i_2}(X_{i_2} - g + g') = v_{i_2}(X_{i_2})$ (from \cref{lem:transfer}). This must belong to some other agent $i_3$. We update $Z$ by moving $g'$ from $i_2$ to $i_3$. We continue this process till we have a sequence of agents (which may repeat) $i_1 \rightarrow i_2 \rightarrow \dots \rightarrow i_r$. Note that all of these agents are a part of $D_i(X)$ since by \cref{lem:transfer} and our construction. To show this it suffices to show that there is a transfer path from $i_1$ to $i_r$ since if there is a path that can increase $i_1$'s utility, this path can be extended to increase $i$'s utility for some $i$ in $S$ since $i' \in D_S(X)$. It is easy to see that giving each $i_p$ the same good in $i_{p+1}$ that was transferred from $Z_{i_p}$ to $Z_{i_{p+1}}$ for all $p \in [r-1]$ is a valid transfer path from $i_1$ to $i_r$.

We stop the sequence if the allocation after the transfer is Pareto dominant for the set of agents $D_i(X)$. This would create a Pareto dominant allocation $Z$ with $\sum_{j \in N \cup \{0\}} |X_j \cap Z_j| > \sum_{j \in N \cup \{0\}} |X_j \cap Y_j|$ --- a contradiction. Note that the sequence has to be finite because it will end when all the agents in $D_i(X)$ have the same bundles as they did in $X$. However note that this is not possible since there are goods that agents in $D_i(X)$ have in $Y$ that they do not have in $X$. We do not transfer goods to agents outside $D_i(X)$. So this would mean the goods just disappeared which is a contradiction. 
\end{proof}
\fi

\if 0
\subsection{Correctness}
\begin{prop}\label{prop:transfer-path-concat}
Let $X = X_0,\dots,X_n$ be some allocation. If there is a transfer path from $j$ to $0$, and $j\in D_i(X)$, then there is a transfer path from $i$ to $0$
\end{prop}
\begin{proof}
 Let us first consider the case where the two transfer paths do not share any intermediate players. Since $j\in D_i(X)$, there is some transfer path from $i$ to $j$, where $j$ loses some item $g$. Since there is a transfer path from $j$ to $0$, then there is a sequence of transfers ending with $0$ such that $j$ gains an item $g'$ for which $\Delta_j(X_j,g') = 1$. Now, since $v_j$ is an MRF, $1 =\Delta_j(X_j,g') \le \Delta_j(X_j\setminus \{g\},g')$, thus $\Delta_j(X_j\setminus\{g\},g') = 1$. In other words, if we concatenate the transfer path from $i$ to $j$, and the transfer path from $j$ to $0$, we obtain a valid transfer path from $i$ to $0$. 
 
Let us next consider the case where there is a single agent $k\ne j,i,0$ who appears in both the transfer path from $i$ to $j$, and from $j$ to $0$. 
Let $(i,p_1,\dots,p_r,k,p_{r+1},\dots,p_s,j)$ be the transfer path from $i$ to $j$, and let $(j,q_1,\dots,q_t,k,q_{t+1},\dots,q_u,0)$ be the transfer path from $j$ to $0$ (any of the sub-paths under this notation can be empty with no change to the proof). 
Suppose that under the transfer path from $i$ to $j$, $k$ loses the item $c$, and under the transfer path from $j$ to $0$, $k$ loses the item $d$. 
If $c = d$, then $(i,p_1,\dots,p_r,k,q_{t+1},\dots,q_u,0)$ is a valid transfer path from $i$ to $0$. If $c \ne d$ then we do the following:  
\end{proof}
\begin{lemma}\label{lem:no-0-path-after-flag}
At every iteration after $\flag_i$ is set to \true for some agent $i$, $0 \notin D_i(X)$
\end{lemma}
\begin{proof}
First, $\flag_i$ is set to \true only when there is no path from $0$ to $i$, thus $0 \notin D_i(X)$ immediately following the step where $\flag_i$ is set to \true. We must show that it is impossible that such a path appears due to other agents' item transfers.

Let us consider the first iteration after $\flag_i$ was set to \true, where a path formed from $i$ to agent $0$. 
 Suppose that this is a path of length $1$, i.e. $0$ can now transfer some good $g$ to $i$ that increases $i$'s welfare. The good $g$ was not in $X_0$ before, thus it must be that agent $0$ appeared as an intermediate agent, received $g$ from some agent $j$, who then continued a transfer path ending again in agent $0$. However, this implies that the truncated transfer path $(i,j,\dots,0)$ was available before the current iteration, a contradiction to our assumption that the current iteration is the first where a path formed from $i$ to agent $0$.
The general case is similar. Let us call the newly formed transfer path $(i,p_1,\dots,p_r=0)$, where $g_1$ is received by $i$; $g_2$ is received by $p_1$ and so on, and $g_r$ is given by agent $0$ to $p_{r-1}$. At least one good $g_\ell$ was not in the possession of $p_\ell$ prior to the current iteration, and thus was transferred to $p_\ell$ via some transfer path from some player $j$ that ends at agent $0$. However, this means that $(i,p_1,\dots,p_\ell,j,\dots,0)$ is a valid transfer path that existed prior to the current iteration, a contradiction to our assumption. 
\end{proof}
\begin{lemma}\label{lem:flagged-no-bundle-change}
At every iteration after $\flag_i$ is set to \true under Algorithm \ref{algo:yankee-swap}, the bundle of agent $i$ remains unchanged.
\end{lemma}
\begin{proof}
The only way that an agent's bundle can change is if they are a part of a transfer path that ends at $0$. Let us consider the first iteration where agent $i$'s bundle changes. If $i$'s bundle has changed, then this means that there is some player $j$ that initiated a transfer path including $i$, which terminates at $0$. However, this in particular means that player $i$ has a transfer path that ends at $0$ as well, a contradiction to Lemma \ref{lem:no-0-path-after-flag}.
\end{proof}
\begin{lemma}\label{lem:no-new-agents-D-i}
At every iteration after $\flag_i$ is set to \true, no new transfer paths starting at $i$ form.  
\end{lemma}
\begin{proof}
Let $X = (X_0,X_1,\dots,X_n)$ be the allocation when $\flag_i$ was set to \true, . 
Let $j$ be  the first agent that $i$ formed a new transfer path to during the run of Algorithm \ref{algo:yankee-swap}, after $\flag_i$ was set to \true. Let us call the allocation at that time $Y=(Y_0,Y_1,\dots,Y_n)$. 

We first analyze the case where there is a direct path from $i$ to $j$, i.e. under $Y$ there is some good $g \in Y_j$ such that $\Delta_i(Y_i,g) = 1$. By Lemma \ref{lem:flagged-no-bundle-change}, $Y_i = X_i$, i.e. $\Delta_i(X_i,g) = 1$. In order to have player $j$ receive $g$, there must have been some transfer path ending at $0$ where $g$ was transferred to $j$; however, this means that $g$ belonged to some other agent $k$, i.e. a transfer path starting at $k$ and ending at $0$ exists, say $(k,p_1,\dots,p_r,0)$. However, this implies that the path $(i,k,p_1,\dots,p_r,0)$ existed in the previous round, a contradiction to Lemma \ref{lem:no-0-path-after-flag}

% Assume this holds at the end of $k$ iterations. After the $k+1$-th iteration, if no transfer was made, then our statement trivially holds. 
% Assume some transfer was made. 
% Assume some transfer path exists either to $0$ or an agent with a bundle of size $ \ge |X_i| + 2$. Let $j \rightarrow j'$ be the first edge which disagrees with the transfer paths of $i$ under the allocation $X$ --- there has to be at least one.
% This edge must disagree because $j$ wants a good from $j'$ that $j'$ did not have before. Let's call this good $g$. 
% At the start of the iteration $g$ must have belonged to some other agent, say $j''$. Thus, there must be a path from $i$ to $j''$, and a path from $j''$ to $0$ where $j''$ got rid of the good $g$. This is based on the fact that $j''$ was a part of the transfer path used in the iteration and in that transfer path $j''$ gave up the good $g$ to obtain another good and retain its bundle size and utility.

\end{proof}
\begin{lemma}\label{lem:size-upper-bound}
At every iteration of Algorithm \ref{algo:yankee-swap}, for every $i\in N$ and every agent $j$ in $D_i(X)$, $|X_j|\le |X_i|+1$.
\end{lemma}
\begin{proof}
Suppose that $j\in D_i(X)$ has an allocation such that $|X_j| \ge |X_i|+2$. When Algorithm \ref{algo:yankee-swap} 
Let us consider the iteration of Algorithm \ref{algo:yankee-swap} where the size of $X_j$ grows from $|X_i|+1$ to $|X_i|+2$. The only way that agents' bundles grow is if they initiate a transfer path. Agent $i$'s welfare is lower than $j$'s; furthermore, $\flag_i=\false$: there is a transfer path from $j$ to $0$, and one from $i$ to $j$ and in particular, there is a transfer path from $i$ to $0$ as per Proposition \ref{prop:transfer-path-concat}. Thus, it cannot be that $j$ was selected to receive an item prior to $i$ at that iteration, since Algorithm \ref{algo:yankee-swap} always selects agents with smaller bundles to initiate transfers, and $|X_j|=|X_i|+1> |X_i|$. 

Finally, it is impossible that $j$ joins $D_i(X)$ after $\flag_i$ is set to \true, as per Lemma \ref{lem:no-new-agents-D-i}.   

\end{proof}
% \begin{remark}
% The above proof must be modified slightly when we replace transfers along paths with swaps using matroid intersection. My guess is that it still works.
% \end{remark}
\begin{theorem}
\cref{algo:yankee-swap} terminates in a non-redundant leximin allocation.
\end{theorem}
\begin{proof}
Let $X = X_0,X_1,\dots,X_n$ be the output of Algorithm \ref{algo:yankee-swap}.
Assume for contradiction that it does not terminate in a leximin solution. Let $Y$ be a leximin solution that maximally intersects with $X$ i.e. $\sum_{j \in N \cup \{0\}} |Y_j \cap X_j|$. Let $i$ be the agent with the lowest utility that $Y$ provides higher utility to, and let $u = v_i(X_i) = |X_i|$. Let $S$ be the set of all $j \in N$ with size $u$. 
We have, from Proposition \ref{prop:demand-set-optimal} that no allocation can provide a higher USW for $D_S(X)$. Therefore, we have $\sum_{j \in D_S(X)} v_j(Y_j) \le \sum_{j \in D_S(X)} v_j(X_j)$. 

If $Y$ has the same number of agents with utility $u$ as $X$, then there exists an agent (say $i_1$) such that $u = |Y_{i_1}| < |X_{i_1}|$. 
Using the matroid exchange property, there must be some good $g_1 \in X_{i_1} \setminus Y_{i_1}$ such that $\Delta_{i_1}(Y_{i_1},g_1) = 1$. 
Let this good belong to another agent $i_2$. Similarly, if, $|Y_{i_2}| \le |X_{i_2}|$ there exists some good $g_2 \in X_{i_2} \setminus Y_{i_2}$ such that $\Delta_{i_2}(Y_{i_2}, g_2)=1$. 
We continue this sequence until we reach an agent $i_r$ such that $|Y_{i_r}| > |X_{i_r}|$. Therefore, we have a sequence of agents $i_1,i_2,\dots,i_r$, such that $|Y_{i_r}| > |X_{i_r}|$. If $|Y_{i_r}| > u+1$, then we can transfer backwards along this path from $i_r$ to $i_1$, to create an allocation that lexicographically dominates $Y$, a contradiction. 
If $|Y_{i_r}| \le u$, then from $|Y_{i_r}| > |X_{i_r}|$, we get that $i_{r}$ has utility $\le u -1$ and $Y$ provides higher utility to $i_r$ contradicting our choice of $i$. If $|Y_{i_r}| = u+1$, we can transfer along the path $i_1 \rightarrow i_2 \rightarrow \dots \rightarrow i_r$ such that at each transfer we give an agent a good they had in $X$ and remove a good they did not have in $X$. This transfer creates an allocation $Z$ with the same utility vector as $Y$ but has a higher intersection with $X$ i.e. $\sum_{j \in N \cup \{0\}} |Z_j \cap X_j| >  \sum_{j \in N \cup \{0\}} |Y_j \cap X_j|$ --- again, a contradiction.

If $Y$ has fewer agents with utility $u$, then at least one of the agents in $S$ must have higher utility in $Y$ than in $X$. However since $\sum_{j \in D_S(X)} v_j(Y_j) \le \sum_{j \in D_S(X)} v_j(X_j)$, some agents in $D_S(X)$ must have lower utility in $Y$ than in $X$. Due to \cref{lem:size-upper-bound}, these agents must have a bundle of size $u+1$ in $X$ and a bundle of size $u$ in $Y$. If any of these agents have a bundle of size $\le u$ in $X$ and $\le u-1$ in $Y$, it is easy to see that $X$ lexicographically dominates $Y$ contradicting the assumption that $Y$ is leximin.
Therefore, for every additional unit of utility that an agent of size $u$ gains in $Y$, there exists an agent who does not have a size $u$ bundle in $X$ but does have a size $u$ bundle in $Y$. This means that there cannot be fewer agents with a bundle of size $u$ in $Y$. Therefore, $X$ is in fact leximin.
\end{proof}
\fi 

==> eit.tex <==
\section{Warm-Up: Envy-Induced Transfers}\label{sec:EIT-simple}
\cite{benabbou2021MRF} propose the following algorithm for computing EF-1 and USW maximizing allocations under MRF valuations. First, compute a USW optimal allocation (using matroid intersection algorithms); next, while there exists any envy beyond one good between any two agents, transfer an item from the envied agent to the envious agent (the existence of an item that will increase the envious agent's utility in the envied agent's bundle is guaranteed since valuations are submodular). 

This algorithm carries two benefits over \citet{Babaioff2021Dichotomous}'s method: it is both simpler to implement, and runs faster. 

We begin by presenting a further simplification of \citeauthor{benabbou2021MRF}'s method: rather than transferring items only between envious agents, we transfer items whenever the gap in valuations exceeds 2. More formally, a \emph{valid transfer} between agents $i$ and $j$ is one where $j$ can get a positive marginal gain from one of the items in $i$'s bundle, and $i$'s utility exceeds $j$'s utility by more than $1$.


\begin{algorithm}
    \caption{Computing an USW+EF-1 allocation for MRFs }
    \label{algo:EIT-algorithm}
    \begin{algorithmic}
        \State $X = (X_1, \dots, X_n) \gets \texttt{ComputeCleanOptimalAllocation}(G,v_1,\dots,v_n)$
        \State $\flag \gets \true$
        \While{$\flag =\true$}
        \State $\flag \gets \false$
        \For{$j \in N$ sorted from highest utility to lowest utility agent}
            \For{$i \in N$ sorted from lowest utility to highest utility agent}
                \If{$\exists g \in X_j$ such that $\Delta_i(X_i,g) = 1$ and $v_j(X_j) > v_i(X_i) + 1$}
                    \State $X_i \gets X_i \cup \{g\}$
                    \State $X_j \gets X_j \setminus \{g\}$
                    \State $\flag \gets \true$
                \EndIf
            \EndFor
        \EndFor
        \EndWhile
        \State \Return $(X_1,\dots,X_n)$
    \end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:EIT-simplified}
Algorithm \ref{algo:EIT-algorithm} outputs an EF-1 and USW optimal allocation.
\end{theorem}
\begin{proof}
Algorithm \ref{algo:EIT-algorithm} starts with an optimal item allocation. At every round, an agent loses an item (and therefore their utility decreases by $1$), and another gains an item that they have positive marginal benefit for (and therefore their utility increases by $1$). Thus, the overall welfare of the allocation is unchanged by the transfers. 

Next, we observe that we continue transferring items from ``rich'' agents to ``poor'' agents as long as the differences in their utilities is more than 1. Suppose that agent $i$ envies agent $j$ for more than one good, i.e. $v_i(X_i)+1 < v_i(X_j)$. The allocation is initially clean, and remains clean at every iteration, since \begin{inparaenum}[(a)]
\item we always give items to agents that gain from receiving them, and
\item when we take an item from an agent, their utility must decrease by $1$ (or else we did not start with a USW optimal allocation). 
\end{inparaenum}   
Since agent valuations have binary gains, $v_j(X_j) = |X_j|$, and $v_i(X_i) = |X_i|$. Furthermore, since agent valuations are submodular, $v_i(X_j) \le |X_j|$. Putting these together we have that
\begin{align*}
    v_i(X_i)+1 < v_i(X_j) &\Rightarrow v_i(X_i)+1 < |X_j| = v_j(X_j)
\end{align*}
Thus, $v_j(X_j)>v_i(X_i)+ 1$. Furthermore, as shown by \citeauthor{benabbou2021MRF}, under MRF valuations, if $i$ envies $j$, there is some item $g$ in $j$'s bundle such that $\Delta_i(X_i,g) = 1$. 
We conclude that Algorithm \ref{algo:EIT-algorithm} does not terminate as long as some agent envies another for more than one good. 

Finally, Algorithm \ref{algo:EIT-algorithm} terminates in polynomial time due a similar potential function argument made in \cite{benabbou2021MRF}: if we transfer an item from $j$ to $i$ and $v_i(X_i) +1 < v_j(X_j)$, the potential function $\sum_{i = 1}^n v_i(X_i)^2$ strictly decreases. 
\end{proof}
The proof of Theorem \ref{thm:EIT-simplified} does not make use of the fact that we first enact feasible item transfers from the most well-off agents to the least well-off agents. However, doing so does result in more efficient transfers. 
\begin{example}
Consider a setting with three agents with binary additive utilities, and $6k$ identical items desired by all agents. We start with the optimal allocation assigning all items to agent 3. A naive item transfer protocol might first transfer items from agent 3 to agent 2 until both have $3k$ items (a total of $3k$ iterations), and then transfer $k$ items from agent 2 to agent 1, and another $k$ items from agent 3 to agent 1 (for $2k$ additional iterations). This results in a total of $5k$ transfers. However, following Algorithm \ref{algo:EIT-algorithm} will have agent 3 alternate item transfers between agents 1 and 2 until all agents have exactly $2k$ items, for a total of $4k$ transfers.
\end{example}
Transferring items between disparate agents, regardless of their envy, is also a good way of balancing non-egalitarian outcomes. 
\begin{example}
Consider the case of two agents, where agent 1 only wants apples and agent 2 wants either apples or bananas. We have one apple and one banana. Assigning both the apple and the banana to agent 2 is a socially optimal outcome; furthermore, since agent 1 only wants the apple, this is an EF-1 outcome as well. Thus, \citeauthor{benabbou2021MRF}'s algorithm will terminate and output this allocation. However, Algorithm \ref{algo:EIT-algorithm} will transfer the apple from agent 2 to agent 1, resulting in a utility of 1 to both agents.  
\end{example}

While Algorithm \ref{algo:EIT-algorithm} is somewhat simpler than \citeauthor{benabbou2021MRF} and \citeauthor{Babaioff2021Dichotomous}'s proposed methods, it still suffers from two major shortcomings. First, single item transfers may not achieve a leximin outcome (see Example \ref{ex:single-transfers-break}); secondly, it still requires one to first compute an optimal allocation, and then correct envy issues via item transfers.

\begin{example}\label{ex:single-transfers-break}
We have three agents, $1,2$ and $3$, and five items, four apples ($a$) and one banana ($b$). The current allocation is as follows: 
$$X_1 = \emptyset; X_2 = \{a,b\}; X_3 = 3\times a.$$
In other words, agent 3 has three apples, agent 2 has an apple and a banana, and agent 1 has nothing. Agents have binary additive valuations, where agent 1 only wants bananas, agent 2 wants either apples or bananas, and agent 3 wants only apples. 
The current allocation is efficient and EF-1: agent 1 is the only envious agent, and desires agent 2's banana. In addition, any single item transfer will not result in an EF-1 and efficient allocation: giving the banana to agent 1 makes agent 2 envy agent 3's abundance of apples. However, we can transfer items along a path: agent 3 gives one apple to agent 2, who in turn gives a banana to agent 1. The resulting allocation is lexmin and envy-free.   
\end{example}
